CONFIG: Constrained Efficient Global Optimization for Closed-Loop Control System Optimization with Unmodeled Constraints

In this paper, the CONFIG algorithm, a simple and provably efficient constrained global optimization algorithm, is applied to optimize the closed-loop control performance of an unknown system with unmodeled constraints. Existing Gaussian process based closed-loop optimization methods, either can only guarantee local convergence (e.g., SafeOPT), or have no known optimality guarantee (e.g., constrained expected improvement) at all, whereas the recently introduced CONFIG algorithm has been proven to enjoy a theoretical global optimality guarantee. In this study, we demonstrate the effectiveness of CONFIG algorithm in the applications. The algorithm is first applied to an artificial numerical benchmark problem to corroborate its effectiveness. It is then applied to a classical constrained steady-state optimization problem of a continuous stirred-tank reactor. Simulation results show that our CONFIG algorithm can achieve performance competitive with the popular CEI (Constrained Expected Improvement) algorithm, which has no known optimality guarantee. As such, the CONFIG algorithm offers a new tool, with both a provable global optimality guarantee and competitive empirical performance, to optimize the closed-loop control performance for a system with soft unmodeled constraints. Last, but not least, the open-source code is available as a python package to facilitate future applications.

==> building_ex.tex <==
\subsection{Batch performance optimization: building controller tuning}
In this section, we consider a room temperature controller tuning problem. We use \textsf{Energym}~\cite{scharnhorst2021energym} with a lower level \textsf{EnergyPlus}~\cite{crawley2001energyplus} model as our building simulator. We consider a bang-bang controller controlling the temperature of an apartment and tune two tolerance thresholds for temperature deviation from predefined temperature set-points. Our objective is to minimize the energy consumption of the apartment while keeping the average temperature deviation below a given threshold. Our problem is formulated as in Eq.~\eqref{eqn:build_formulation}.
\bse\label{eqn:build_formulation}
\begin{align}
\min_{\theta\in\Theta}  \qquad& J(\theta) \\
\text{subject to} \qquad & g(\theta)-g_{\mathrm{thr}}\leq 0,\quad
\end{align}
\ese
where $J(\theta)$ represents energy consumption in this example, $g(\theta)$ represents average temperature deviation and $g_\mathrm{thr}$ is a given average temperature deviation threshold. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{ifacconf_latex/figs/energym_case.pdf}
    \caption{Demonstration of building temperature controller tuning.}
    \label{fig:building_tune_ex}
\end{figure}

Fig.~\ref{fig:building_tune_ex} demonstrates the overall solution of applying our constrained efficient global optimization algorithm to the building temperature controller tuning problem. In each step, our algorithm selects a set of promising controller parameters. We use this set of parameters to run a closed-loop building simulation over a period of $1$ day, using an \textsf{EnergyPlus}~\cite{crawley2001energyplus} simulator of a building located in Spain, Tarragona. In this case study, the objective and the constraints are expensive functions in that each round of closed-loop simulation over the period of one day can take more than 15 minutes on an \textsf{Intel(R) Core(TM) i7-10610U CPU @ 1.80GHz} machine.

Based on the closed-loop trajectory, we calculate the key performance indicators, that is, energy consumption and average temperature deviation. We then update the Gaussian process regression with the new data added.  
\begin{figure}
    \centering
    \includegraphics{ifacconf_latex/figs/building_funcs_r_and_v.pdf}
    \caption{Best normalized energy consumption plus normalized temperature deviation up to current step. For \textsf{SafeOPT}, the initial required feasible solution is obtained based on domain knowledge.}
    \label{fig:best_normalized_energy_plus_dev}
\end{figure}

Since energy consumption and temperature deviations are in two different scales, we use normalized energy consumption $\frac{J}{\sigma_J}$ plus normalized average temperature deviation $\frac{[g-g_\mathrm{thr}]^+}{\sigma_g}$ to measure the quality of the solution, where $\sigma_J, \sigma_g$ are standard deviations determined from a set of randomly sampled solutions.   Fig.~\ref{fig:best_normalized_energy_plus_dev} gives the best normalized energy consumption plus average temperature deviation up to the current step. We observe that within $20$ steps, our algorithm identifies the solution with minimum normalized energy consumption plus normalized average temperature deviation, verifying the competitiveness of our algorithm with the currently popular constrained expected improvement method again. In contrast, the SafeOPT method can be overly cautious, and fails to find a solution with performance comparable to the CEI method or to ours. 
